The uniqueness of Lyapunov rank among symmetric cones

The Lyapunov rank of a cone is the dimension of the Lie algebra of its automorphism group. It is invariant under linear isomorphism and in general not unique - two or more non-isomorphic cones can share the same Lyapunov rank. It is therefore not possible in general to identify cones using Lyapunov rank. But suppose we look only among symmetric cones. Are there any that can be uniquely identified (up to isomorphism) by their Lyapunov ranks? We provide a complete answer for irreducible cones and make some progress in the general case.

==> GNUmakefile <==
#
# Example makefile using mjotex and a BibTeX references database.
#
# After defining $(PN) to be the name of your document, this will
# compile the source file $(PN).tex to $(PN).pdf.
#
# To support workflows where the document is kept open in a PDF reader
# during recompilation, the build process takes place in a separate
# $(BUILDDIR) directory that defaults to "build". Only when the build
# has completed do we move the resulting $(PN).pdf to the current
# directory. This avoids renaming or modifying the open document in
# place, which in turn helps prevent flickering, loss of bookmarks, et
# cetera, in several PDF readers.

# The build directory. Not broken? Don't fix.
BUILDDIR=build

# The latex compiler. The SOURCE_DATE_EPOCH=0 prevents the creation
# and modification dates from being embedded as metadata into the
# output file; that in turn is important because it allows us to tell
# when the output stops changing (that is, when we are done). The
# variable is supported in pdftex v1.40.17 and later.
LATEX = SOURCE_DATE_EPOCH=0 pdflatex -file-line-error -halt-on-error --output-directory $(BUILDDIR)

# The name of this document.
#
# For example, to use the name of our parent directory:
#
# PN = $(notdir $(realpath .))
#
PN = the_uniqueness_of_lyapunov_rank_among_symmetric_cones

# A space-separated list of bib files. These must all belong to paths
# contained in your $BIBINPUTS environment variable.
#
# Leave commented if you don't use a bibliography database.
#
BIBS = local-references.bib

# A space-separated list of the mjotex files that you use. The path to
# mjotex must be contain in your $TEXINPUTS environment variable.
#
# MJOTEX  = mjotex.sty
#
MJOTEX  = mjo-algebra.tex mjo-arrow.tex mjo-common.tex mjo-cone.tex
MJOTEX += mjo-font.tex mjo-hurwitz.tex mjo-linear_algebra.tex
MJOTEX += mjo-proof_by_cases.tex mjo-set.tex mjo-theorem.tex mjo.bst

# Use kpsewhich (from the kpathsea suite) to find the absolute paths
# of the bibtex/mjotex files listed in in $(BIBS)/$(MJOTEX). The SRCS
# variable should contain all (Bib)TeX source files for the document.
SRCS = $(PN).tex
SRCS += $(BIBS)
SRCS += $(MJOTEX)

# The first target is the default, so put the PDF document first.
#
# This voodoo is all designed to find a "fixed point" of calling
# $(LATEX). When you build a LaTeX document, it requires an unknown
# number of compilation passes. How do you know when to stop? Easy,
# stop when the output file stops changing! But how to encode that
# in a makefile?
#
# At the start of this rule, we call $(LATEX) to compile $(PN).tex.
# It stores the resulting PDF in a separate "build" directory, so this
# will not actually create or overwrite the target $(PN).pdf. If there
# is no $(PN).pdf already, then we rename the new one to $(PN).pdf and
# we are done. But if there was a previous version, then we compare
# the two (new & old) versions. In either case, we rename the new one
# over the old one. But if the two differ, then we repeat this process
# in a loop until the just-built PDF is identical to the one from the
# previous iteration.
$(PN).pdf: $(SRCS) $(BUILDDIR)/$(PN).bbl $(INDEX_DSTS)
	$(LATEX) $(PN).tex

	if [ -f $@ ]; then \
	  while ! cmp -s $@ $(BUILDDIR)/$(PN).pdf; do \
	    mv $(BUILDDIR)/$(PN).pdf $@; \
	    $(LATEX) $(PN).tex; \
	  done; \
	fi;

	if grep -q 'Rerun to get' $(BUILDDIR)/$(PN).log; then \
	  $(LATEX) $(PN).tex; \
	fi;

	mv $(BUILDDIR)/$(PN).pdf $@

$(BUILDDIR):
	mkdir $@

$(BUILDDIR)/$(PN).aux: $(SRCS) | $(BUILDDIR)
	$(LATEX) $(PN).tex


# The pipe below indicates an "order-only dependency" on the aux file.
# Without it, every compilation of $(PN).tex would produce a new
# $(PN).aux, and thus $(PN).bbl would be rebuilt. This in turn causes
# $(PN).pdf to appear out-of-date, which leads to a recompilation of
# $(PN).tex... and so on. The order-only dependency means we won't
# rebuild $(PN).bbl if $(PN).aux changes.
#
# As a side effect, we now need to depend on $(SRCS) here, since we
# won't pick it up transitively from $(PN).aux.
#
# If the $BIBS variable is undefined, we presume that there are no
# references and create an empty bbl file. Otherwise, we risk trying
# to run biblatex on an aux file containing no citations. If you do
# define $BIBS but don't cite anything, you'll run into a similar
# problem. Don't do that.
#
$(BUILDDIR)/$(PN).bbl: $(SRCS) | $(BUILDDIR)/$(PN).aux
ifdef BIBS
	bibtex $(BUILDDIR)/$(PN).aux
else
	printf '' > $@
endif

# If the output PDF exists but the log file does not, then an attempt
# to "build the log file" (i.e. build the PDF) would do nothing. Thus
# whenever the log file does not exist, we do a fresh build.
$(BUILDDIR)/$(PN).log: $(SRCS)
	$(MAKE) clean
	$(MAKE)

# Ensure that there are no overfull or underfull boxes in the output
# document by parsing the log for said warnings.
.PHONY: check-boxes
check-boxes: $(BUILDDIR)/$(PN).log
	@! grep -i 'overfull\|underfull' $<

# Run chktex to find silly mistakes. There is some exit code weirdness
# (Savannah bug 53129), so we just look for empty output.
.PHONY: check-chktex
CHKTEX = chktex --localrc .chktexrc --quiet --inputfiles=0
check-chktex:
	@chktexout=$$($(CHKTEX) $(PN).tex); \
	  test -z "$${chktexout}" || { echo "$${chktexout}" 1>&2; exit 1; }

# Ensure that there are no undefined references in the document by
# parsing the log file for said warnings.
.PHONY: check-undefined
check-undefined: $(BUILDDIR)/$(PN).log
	@! grep -i 'undefined' $<

# Run python doctests
.PHONY: check-python
check-python:
	cd tests && python -m doctest ./*.py && cd ../

# Run a suite of checks.
.PHONY: check
check: check-boxes check-chktex check-undefined check-python

# Clean up leftover junk. This only looks overcomplicated because
# the *.{foo,bar} syntax supported by Bash is not POSIX, and Make
# will execute these commands using /bin/sh (which should be POSIX).
JUNK_EXTENSIONS  = aux bbl bcf blg glo ilg ist listing lof log nav out pdf
JUNK_EXTENSIONS += snm spl toc xml
.PHONY: clean
clean:
	for ext in $(JUNK_EXTENSIONS); do rm -f *.$$ext; done;
	rm -rf dist/ $(BUILDDIR)/
	rm -f $(SAGE_LISTING_DSTS) $(INDEX_SRCS) $(INDEX_DSTS)

# If this document will be published, the publisher isn't going to
# have your BibTeX database or your mjotex files. So, you need to
# package them up along with the code for your document. This target
# will create a "dist" directory and copy the necessary stuff there.
#
.PHONY: dist
dist: $(BUILDDIR)/$(PN).bbl
	mkdir -p dist
	cp $(SRCS) dist/


